Reinforcement Learning-based Approach for Vehicle-to-Building Charging with Heterogeneous Agents and Long Term Rewards

Strategic aggregation of electric vehicle batteries as energy reservoirs can optimize power grid demand, benefiting smart and connected communities, especially large office buildings that offer workplace charging. This involves optimizing charging and discharging to reduce peak energy costs and net peak demand, monitored over extended periods (e.g., a month), which involves making sequential decisions under uncertainty and delayed and sparse rewards, a continuous action space, and the complexity of ensuring generalization across diverse conditions. Existing algorithmic approaches, e.g., heuristic-based strategies, fall short in addressing real-time decision-making under dynamic conditions, and traditional reinforcement learning (RL) models struggle with large state-action spaces, multi-agent settings, and the need for long-term reward optimization. To address these challenges, we introduce a novel RL framework that combines the Deep Deterministic Policy Gradient approach (DDPG) with action masking and efficient MILP-driven policy guidance. Our approach balances the exploration of continuous action spaces to meet user charging demands. Using real-world data from a major electric vehicle manufacturer, we show that our approach comprehensively outperforms many well-established baselines and several scalable heuristic approaches, achieving significant cost savings while meeting all charging requirements. Our results show that the proposed approach is one of the first scalable and general approaches to solving the V2B energy management challenge.

==> figures/symbols.tex <==
\begin{table}[t]
    \centering
    \small
    \caption{Key symbols.}
    \begin{tabular}{|p{1.8cm}|p{6.0cm}|}
    \hline
    \textbf{Notation} & \textbf{Description} \\
    \hline
    $\mathcal{C}=\{C^i\}$ & Set of chargers, where each charger is $C^i$ \\ \hline
    ${\it P}^i_{min}, {\it P}^i_{max}$ & Minimum and maximum power rates of charger $C^i$ (kW) \\ \hline
    $\mathcal{T}$, $\mathcal{T}_{P}$ & Time slots during billing period and peak hours (minutes) \\ \hline
    % $\mathcal{T}_{P}$ &  \\ \hline
    $\Delta t $ & The time interval for charging control (hours) \\ \hline 
    $v$,  $v_t^i$& an EV and the EV connected to charger $C^i$ at time $t$  \\ \hline
    $P^i_t$ & Charging power of charger $C^i$ at time $t$ (kW) \\ \hline
    ${\it SoC}^{req}(v)$ & Required SoC for EV $v$ (\%) \\ \hline
    ${\it SoC}^{in}(v)$ & Initial SoC of EV $v$ at arrival (\%) \\ \hline
    ${\it SoC}_t(v)$ & SoC of EV $v$ at time $t$ (\%) \\ \hline
    ${\it SoC}^{min}(v)$, ${\it SoC}^{max}(v)$ & Minimum and maximum SoC ratio boundaries of EV $v$ (\%) \\ \hline
    ${\it Cap}(v)$ & Energy capacity of EV $v$ (kWh) \\ \hline
    $T_d(v), T_a(v)$ & Departure and arrival times of EV $v$ (minutes) \\ \hline
    % ${\it V2C}(v)$ & Charger assigned to EV $v$ \\ \hline
    ${\it Pr}^{E}_t$, ${\it Pr}^{D}$ & Electricity price at time $t$ and Demand price (\$/kWh, \$/kW) \\ \hline
    $B_t$ & Building load at time $t$ (kW) \\ \hline
    $ B^{hist}_t$ & List of previous seven days' peak building loads (kW) \\ \hline
    ${\it Arr}^{EV}_t$ & Cumulative EV arrivals by time $t$ (number of EVs) \\ \hline
    ${\it Pk}^{prd}_t$ & Predictive peak power at time $t$ (kW) \\ \hline 
    $\mathcal{\it CS}_{t}$ & EV status across chargers $ \mathcal{C} $ at time $t$ \\ \hline
    $s_t$ & State at time step $t$ \\ \hline
    $a_t$ & Action at time step $t$ \\ \hline
    $\pi(s_t)$ & RL policy function \\ \hline
    $\lambda_{SoC}$, $\lambda_{Bill}$, $\lambda_{DC}$ & Penalty coefficients for SoC requirement, bill cost, and demand charge \\ \hline
    \end{tabular}
    \label{table:notations}
\end{table} 

==> results/charger_assignments.tex <==


\pgfplotstableread[col sep=comma]{charger_assignments.csv}{\chargerassignments}

\begin{table}[htp]
\centering
\caption{Charger Assignment and tiebreaker comparisons with an MILP policy. Assigning to Bidirectional chargers first and then breaking ties by assigining them to the EV that departs later results in the lowest bill. Lower is better.}
\pgfplotstabletypeset[
    create on use/bill/.style={
        create col/assign/.code={%
            \edef\entry{\thisrow{c}$\pm$\thisrow{d}}
            \pgfkeyslet{/pgfplots/table/create col/next content}{\entry}
        }
    },
    columns ={a, b, bill},
    column type=c,
    columns/a/.style={string type},
    columns/b/.style={string type,column type=c},
    columns/bill/.style={string type,column type=c},
    fixed,
    fixed zerofill,
    precision=2,
    every head row/.style={
        output empty row,
        before row={%}
            \toprule
            {Assignment} & {Tie Breaker} & {Average Monthly Bill (\$)}\\
        }, 
        after row=\midrule},
    every last row/.style={after row=\bottomrule},
    every row 0 column 0/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 0 column 1/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    % every row 0 column 2/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    % every row 0 column 3/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    ] {\chargerassignments}
\label{table:charger_assignment_policies}
\end{table}



==> results/month_demand_charge.tex <==


% ,policy,episode_name,total_building_energy_used_kWh,total_charge_to_cars_kWh,total_discharge_to_cars_kWh,max_demand_pw_15min_kW,demand_charge_cost_usd,total_elec_cost_usd,total_bldg_cost_usd,total_bill_usd,total_energy_needed_from_arrive_to_rsoc_kWh,total_missing_charge_upon_depart_kWh,total_excess_charge_upon_depart_kWh,num_cars_not_at_rsoc_upon_depart_count,heuristic_threshold,time_before_heuristics,sample,month
% 0,NO_CHARGING,./data/input_csvs/9_8_month_test/AUG2023/45_827,51159.73,0.0,0.0,225.10434933959897,2165.503840646942,0.0,7218.271225707637,9383.77506635458,892.03,892.03,0.0,156,None,3600,45_827,AUG2023 
\pgfplotstableread[col sep=comma]{testdata.csv}{\demandshavetable}

\begin{table*}[h]
\centering
\caption{Comparison of peak shaving for the evaluation set, best values are bold. MILP shows the optimal solution given an oracle input. Higher is better.}
\pgfplotstabletypeset[
    % dec sep align=S,    % Use the siunitx `S` column type for aligning at decimal point
    fixed,fixed zerofill,     % Fill numbers with zeros
    precision=2,        % Set number of decimals
      columns/Policy/.style={
        string type,
        postproc cell content/.code={%
            \pgfplotsutilstrreplace{_}{\_}{##1}%
            \pgfkeyslet{/pgfplots/table/@cell content}\pgfplotsretval
        },
      },
     columns/Month/.style={
        string type,
        postproc cell content/.code={%
            \pgfplotsutilstrreplace{_}{\_}{##1}%
            \pgfkeyslet{/pgfplots/table/@cell content}\pgfplotsretval
        },
      },
    every head row/.style={before row=\toprule, after row=\midrule},
    every last row/.style={after row=\bottomrule},
    % every even row/.style={before row={\rowcolor[gray]{.8}}}, %Adding row colors
    every first row/.style={before row={\rowcolor[gray]{.8}}},
    every row 1 column 1/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 1 column 2/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 1 column 3/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 1 column 4/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 1 column 5/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 1 column 6/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 1 column 7/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 1 column 8/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 1 column 9/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 1 column 10/.style={numeric type, postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    ] {\demandshavetable}
\label{table:peak_shaving_demand}
\end{table*}

==> results/month_total_bill.tex <==



\pgfplotstableread[col sep=comma]{total_bill.csv}{\totalbilltable}

\begin{table*}[h]
\centering
\caption{Comparison of final total bill on the evaluation, set best values are bold. MILP shows the optimal solution given an oracle input. Lower is better.}
\pgfplotstabletypeset[
    create on use/bill/.style={
        create col/assign/.code={%
            \edef\entry{\thisrow{MAY}$\pm$\thisrow{MAY}}
            \pgfkeyslet{/pgfplots/table/create col/next content}{\entry}
        }
    },
    % dec sep align=S,    % Use the siunitx `S` column type for aligning at decimal point
    fixed,fixed zerofill,     % Fill numbers with zeros
    precision=2,        % Set number of decimals
      columns/Policy/.style={
        string type,
        postproc cell content/.code={%
            \pgfplotsutilstrreplace{_}{\_}{##1}%
            \pgfkeyslet{/pgfplots/table/@cell content}\pgfplotsretval
        },
      },
     columns/Month/.style={
        string type,
        % postproc cell content/.code={%
        %     \pgfplotsutilstrreplace{_}{\_}{##1}%
        %     \pgfkeyslet{/pgfplots/table/@cell content}\pgfplotsretval
        % },
        postproc cell content/.append code={$\pm$ 0.00}, 
      },
    % columns/MAY/.style={postproc cell content/.append code={$\pm$ 0.00}}, 
    % columns/Month/.style={postproc cell content/.append code={$\pm$ 0.00}}, 
    % columns/JUN/.style={postproc cell content/.append code={$\pm$ 0.00}},
    % columns/JULY/.style={postproc cell content/.append code={$\pm$ 0.00}},
    % columns/AUG/.style={postproc cell content/.append code={$\pm$ 0.00}},
    % columns/SEP/.style={postproc cell content/.append code={$\pm$ 0.00}},
    % columns/OCT/.style={postproc cell content/.append code={$\pm$ 0.00}},
    % columns/NOV/.style={postproc cell content/.append code={$\pm$ 0.00}},
    % columns/DEC/.style={postproc cell content/.append code={$\pm$ 0.00}},
    % columns/JAN/.style={postproc cell content/.append code={$\pm$ 0.00}},
    % columns/Total/.style={postproc cell content/.append code={$\pm$ 0.00}},
    every head row/.style={before row=\toprule, after row=\midrule},
    every last row/.style={after row=\bottomrule},
    every first row/.style={before row={\rowcolor[gray]{.8}}},
    every row 1 column 1/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 1 column 2/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 1 column 3/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 1 column 4/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 1 column 5/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 1 column 6/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 1 column 7/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 1 column 8/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 1 column 9/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 1 column 10/.style={postproc cell content/.append style={@cell content={\textbf{##1}}}, zerofill, precision=2,}, 
    ] {\totalbilltable}
\label{table:monthly_total_bill}
\end{table*}

==> results/performance_metrics_training_data.tex <==


\pgfplotstableread[col sep=comma]{performance_metrics.csv}{\perfmetricstable} 
\begin{table*}[htp]
\centering
\caption{Performance Metrics from Equation~(\ref{eq:training_metrice}) of different policies on training data (\%). Lower is better.}
\pgfplotstabletypeset[
    % dec sep align=S,    % Use the siunitx `S` column type for aligning at decimal point
    fixed,fixed zerofill,     % Fill numbers with zeros
    precision=4,     % Set number of decimals
    % display columns/0/.style={
    %     precision=1,    % Change for first column (column index 0)
    %     column name=$\theta_{2,i}$
    % },
    % display columns/1/.style={column name=$X$,column type={S}},
    % display columns/2/.style={column name=$Y$,column type={S}},
    % columns/a/.style={string type},
      columns/Policy/.style={
        string type,
        postproc cell content/.code={%
            \pgfplotsutilstrreplace{_}{\_}{##1}%
            \pgfkeyslet{/pgfplots/table/@cell content}\pgfplotsretval
        },
      },
     columns/Month/.style={
        string type,
        postproc cell content/.code={%
            \pgfplotsutilstrreplace{_}{\_}{##1}%
            \pgfkeyslet{/pgfplots/table/@cell content}\pgfplotsretval
        },
      },
    % every row 0 column 1/.style={string type},
    % every row 0 column 2/.style={string type},
    every head row/.style={before row=\toprule, after row=\midrule},
    every last row/.style={after row=\bottomrule},
    % every first row/.style={before row={\rowcolor[gray]{.8}}},
    every row 0 column 1/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 1 column 2/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 0 column 3/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 0 column 4/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 0 column 5/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 0 column 6/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 0 column 7/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 0 column 8/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 0 column 9/.style={postproc cell content/.style={@cell content={\textbf{##1}}}}, %bolding
    every row 0 column 10/.style={numeric type, postproc cell content/.style={@cell content={\textbf{##1}}}}, 
    ] {\perfmetricstable}
\label{table:performance_metrics_training_data}
\end{table*}
% \FloatBarrier

==> results/simulation_parameter.tex <==
\begin{table*}[htp]
    \centering
    \small 
    \caption{Training and Testing Data Information for Each Month with Simulation Parameters}
    \begin{tabular}{|p{1.0cm}|p{1.5cm}|p{1.7cm}|p{1.7cm}|p{1.0cm}|p{1.0cm}|p{1.5cm}|p{1.7cm}|p{1.7cm}|}
    \hline
    \multirow{2}{*}{\textbf{Month}} & \multicolumn{5}{p{3.75cm}|}{\textbf{Training (60 Samples)}} & \multicolumn{3}{p{3.75cm}|}{\textbf{Testing (50 Samples)}} \\ 
    \cline{2-9} 
    & {Car Arrival Number (per day)} & {Monthly Peak Building Load (kW)} & {Daily Peak Building load (kW)} & {Predicted Peak Power (kW)} & {Weekdays} & {Car Arrival Number (per day)} & {Monthly Peak Building Load (kW)} & {Daily Peak Building Load (kW)} \\ \hline 
    
    \textbf{MAY} & $9.35\pm2.19$ & $125.89\pm1.72$ & $96.22\pm13.76$ & 119 & 22 & $9.31\pm2.2$ & $125.62\pm1.65$ &$96.18\pm13.73$ \\ \hline
    \textbf{JUN} & $11.4\pm2.53$ & $141.04\pm1.83$ & $109.86\pm14.0$ & 125 & 21 & $11.49\pm2.51$ & $140.34\pm2.21$ &$109.75\pm13.97$\\ \hline
    \textbf{JULY} & $10.86\pm2.45$ & $148.08\pm1.57$ & $111.79\pm35.39$ & 145 & 20 & $10.97\pm2.4$ & $148.12\pm1.72$ &$111.94\pm35.49$\\ \hline
    \textbf{AUG} & $6.87\pm1.97$ & $221.02\pm3.86$ & $160.5\pm27.92$ & 202 & 23 & $6.92\pm1.93$ & $221.17\pm3.77$ &$160.69\pm28.14$\\ \hline
    \textbf{SEP} & $14.99\pm2.9$ & $145.91\pm1.48$ & $127.2\pm11.86$ & 143 & 20 & $14.94\pm2.88$ & $146.23\pm1.08$ &$127.2\pm11.85$\\ \hline
    \textbf{OCT} & $14.55\pm2.91$ & $186.54\pm1.72$ & $118.58\pm30.12$& 174 & 21 & $14.54\pm2.86$ &$185.17\pm2.77$ &$118.5\pm30.13$ \\ \hline 
    \textbf{NOV} & $9.59\pm2.31$ & $144.9\pm3.28$ & $113.09\pm19.18$ & 130 & 19 & $9.57\pm2.29$ & $144.2\pm2.92$&  $113.09\pm19.2$\\ \hline 
    \textbf{DEC} & $20.36\pm3.4$ & $116.49\pm2.25$ & $98.72\pm8.0$ & 104 & 16 & $20.32\pm3.35$ & $116.33\pm2.01$ &$98.69\pm7.95$\\ \hline 
    \textbf{JAN} & $13.62\pm2.73$ & $137.77\pm2.47$ & $91.56\pm19.46$ & 127 & 21 & $13.53\pm2.76$ & $137.64\pm2.5$ &$91.72\pm19.47$\\ \hline 
    \end{tabular}
    \vspace{0.5cm}
    \begin{tabular}{|p{3.3cm}|p{9.2cm}|}
    \hline
    \textbf{Parameter} & \textbf{Value} \\
    \hline
    $\mathcal{C}$ & 15 chargers (5 bi-directional, 10 uni-directional) \\\hline
    ${\it P}^i_{min}, {\it P}^i_{max}$ & [-20 kW, 20 kW] for bi-directional, [0, 20 kW] for uni-directional chargers \\\hline
    $\Delta t$ & Time interval: 0.25 hours \\\hline
    $\mathcal{T}$, $\mathcal{T}_P$ & Total time slots in one month, time slots in peak hours (6 am to 10 pm) daily \\\hline 
    $Pr^{D}, Pr^{E}_t$ & 9.62 \$/kW (Demand), 0.11271 \$/kWh (off-peak), 0.1466 \$/kWh (peak) \\\hline
    $Cap(v)$ & EV energy capacity: 40 or 62 kWh \\\hline
    $SoC^{min}(v)$, $SoC^{max}(v)$ & Minimum and maximum SoC: 0\% and 90\% of capacity \\\hline
    \end{tabular}
\end{table*}


==> sections/02_2_MDP.tex <==
\subsection{Markov Decision Process Model}
\label{ssec:MDP}

%We model the V2B problem as a Markov Decision Process (MDP). This framework enables optimal decision-making regarding charger power rates and load management, allowing for effective responses to uncertainties in user behaviors and building loads in our working scenario. 
 % \color{black} We define the MDP as a tuple $(\mathcal{S}, \mathcal{A}, {\it Trans}(S(T_j),A(T_j))$, ${\it Reward}(S(T_j)$, $A(T_j))$, where $\mathcal{S} = \{S(T_j) \mid T_j \in \mathcal{T}\}$ is the set of states representing the system's state at the beginning of each time slot $T_j$, $\mathcal{A} = \{A(T_j) \mid T_j \in \mathcal{T}\}$ is the set of actions, with each action $A(T_j) \in \mathcal{A}$ representing a decision made at time slot $T_j$ and including continuous values indicating the power rate of all chargers. The state transition function $\text{Trans}(S(T_j), A(T_j))$ describes the transition from state $S(T_j)$ to the next state based on action $A(T_j)$, while the reward function $\text{Reward}(S(T_j), A(T_j))$ assigns a reward for taking action $A(T_j)$ in state $S(T_j)$. The key notations in the MDP are provided as follows: 

%We briefly describe the state, actions and transitions for the problem. 
% The key notations in the MDP for the V2B problem are as follows:
% \rishav{add small \\description of MDP, \\as a tuple\\ (S,A,P,T,$\gamma$, \\describing each \\in few words}
%Our objective is to determine the optimal power rate sequence $\mathcal{P}$ across all time slots $T_j \in \mathcal{T}$. 
%To address the uncertainly in our working scenario, we model the V2B problem as a Markov Decision Process (MDP), which effectively tracks changing conditions like fluctuating SoC, building load, and unpredictable EV arrivals. MDPs provide a framework for making optimal decisions regarding charger power rates and load management, ensuring effective responses to variations in user behavior and demand.    We model the V2B charging control process as a MDP, aiming to find the optimal power rate sequence \(\mathcal{P}\) for all time slots \(T_j \in \mathcal{T}\). Our goal is to derive the optimal policy for determining $P(C_i, T_j)$ for each time slot, minimizing the total cost while ensuring that the EVs' SoC requirements are met throughout the billing period.     




{\bf State.}
%At each time slot $T_j\in\mathcal{T}$, we define state $S(T_j) \in \mathcal{S}$ by using a combination of features that we identified through a mix of domain expertise and experiments.
The complete state space for the problem can be described using features that provide historical, current, and future estimation at a given time $T_j$.
%These features provide historical as well as current context and include estimated value of peak power that is used to calculate demand charge.  The complete state features of our V2B problem at each decision-making time 
This includes key input parameters for each vehicle such as the current SoC, required SoC, departure time, and battery capacity for each EV, along with SoC boundaries across 15 chargers. Additionally, the current building load, time slot, day of the week, past historical building load, and long-term peak power estimation value are included, resulting in approximately 100 features. While this state space is complete, it is not tractable to be used for the learning process. Therefore, we had to reduce the state space. For this,
%For improving practical performance, 
we leveraged domain-specific knowledge to abstract key information, reducing the state space to 37 essential state elements without compromising crucial data. We describe them below.
%abstracting the following features providing historical and current building load and arrival EVs, as well as features for future estimation:
    % \item The current building load is $\Building(T_j)$. 
    % \item The power gap between the current builidng load to the estimated peak power for the billing period is $\PrdPeak(T_j) - \Building(T_j)$. By incorporating this long-term peak power estimation, we provide the RL model with a feature that aids in estimating the optimal peak power for demand charge reduction.
    % \item The historical building load information which constrains the mean peak building load$\mu(B^H(T_j))$ and variance $\sigma^2(B^H(T_j))$  over the previous 7 days. This data can also inform estimations of future building load.  
    % \item The current time slot $T_j$ and day of the week are included to help the RL model distinguish daily patterns and manage feature diversity, enhancing generalization across different weekdays. 
    % \item Number of EV arrivals upto time slot $T_j$ for the current day, represented as $|\{V| V\in \mathcal{V}, A(V)\leq T_j \}|$, tracking the current EVs and their status. 
    % \item We include the status of all chargers $\CS(T_j) = \{(\PowerNeed(C_i, T_j)$, $\ReTime(C_i, T_j))\}_{C_i \in \mathcal{C}}$, where each charger status is defined by two components: (i) $\PowerNeed(C_i, T_j)$ representing the energy gap between the required SoC and the current SoC of the EV, where, 
    % \begin{equation*} 
    %  \PowerNeed(C_i, T_j) = ( \SOCR(V) - \SOC(V, T_j) ) \times {\it CAP}(V)
    %  \label{eq:chargerstate}
    % \end{equation*} 
    % with $V=\phi(C_i, T_j)$ indicating the EV connected to $C_i$ at time slot $T_j$
    % and, (ii) $\ReTime(C_i, T_j) = D(\phi(C_i, T_j)) - T_j$, specifying the time remaining till the departure of the EV.
   
    \begin{enumerate}[leftmargin=*]
    \item The current time slot, $T_j$.
    \item The current building load, denoted as ${B}(T_j)$.
    \item The power gap between the current building load and the estimated peak power for the billing period, $ \PrdPeak(T_j) - {B}(T_j)$. It aids the RL model in estimating optimal peak power for demand charge reduction.
    \item The mean peak building load over the previous 7 days, $\mu(B^H(T_j))$.
    \item The variance of the peak building load over the previous 7 days, $\sigma^2(B^H(T_j))$. It informs the model about the future building load.  
    \item The day of the week for the current time slot, $T_j$. It helps the RL model distinguish daily patterns and enhance generalization.
    \item The number of EV arrivals up to time slot $T_j$, represented as $|\{V | V \in \mathcal{V}, A(V) \leq T_j \}|$. This helps in tracking the number of EVs currently present.
    \item The energy needed by each EV that is connected to a charger at time slot $T_j$, given by $[\PowerNeed(C_i, T_j)]_{C_i \in \mathcal{C}}$, and is initialized to $0$. This represents the energy gap between the required SoC and the current SoC of the EV connected to charger $C_i$ at time slot $T_j$, defined as: 
    \begin{equation} 
     \PowerNeed(C_i, T_j) = (\SOCR(V) - \SOC(V, T_j)) \times \text{CAP}(V)
     \label{eq:chargerstate}
    \end{equation}
    where $V=\phi(C_i, T_j)$ indicating the EV connected to $C_i$ at time slot $T_j$. 
    \item The remaining time until the departure of each EV connected to the chargers is given by $[\ReTime(C_i, T_j)]_{C_i \in \mathcal{C}}$, and is set to 0 when no cars are connected. Each term is computed as $\ReTime(C_i, T_j) = \DepartureTime(\phi(C_i, T_j)) - T_j$. 
\end{enumerate} 
   % where $RT(C_i,T_j)$ represents the remaining time before the departure of the EV, i.e.,
    %The energy gap $\PowerNeed(C_i, T_j)$ is calculated based on the difference between the target SoC and the current SoC at time $T_j$.
   % Status of all chargers is given by $\CS(T_j) = \{ CS(C_i, T_j) \}_{C_i \in \mathcal{C}, T_j \in \mathcal{T}}$. Each charger status is specified by $CS(C_i, T_j) = (\PowerNeed(C_i, T_j)$ , $RT(C_i, T_j))$. Here, $\PowerNeed(C_i, T_j)$ represents the energy gap between the required SoC and the current SoC for the EV connected to $C_i$, calculated by: 
 %We set $CS_t^i = (0,0)$ if no EV is connected to charger $C^i$.

% {\bf Initial State.} The initial state $S(T_0)$ is defined at the beginning of the billing period. It consists of the starting building load $B(T_0)= 0$, the estimated peak power $\PrdPeak(T_0)$, which may be derived from historical data or forecasts (as detailed in Section~\ref{ssec:pipeline}), and historical load values from the preceding 7 days, represented as $B^{H}(T_0)$. The initial time is set to $T_0$, corresponding to the day of the week. At this initial time, the number of EV arrivals is $0$. Additionally, all parameters of the initial status of all chargers $\CS(T_0)$ are set to 0.  
%the initial status of all chargers, denoted as $\CS(T_0) = \{ CS(C_i, T_0) \}_{C^i \in \mathcal{C}}$, is initialized with $CS(C_i, T_0) = (0,0)$ for all chargers.  

{\bf Actions.} The actions $A(T_j) \in \mathcal{A}$ in this MDP are continuous and specify the power rates of all chargers at time $T_j$, where $A(T_j) = [P(C_i, T_j)]_{C^i \in \mathcal{C}}$.

{\bf State Transition.} We utilize a discrete event simulator to track the state transitions. \ad{Need to write a bit about the simulator.} The simulator is given a ``chain'' empirically sampled from the data provided by our partner representing a day in the monthly billing period. 
\jpt{Will connect it to the new subsection in Approach}
Each chain is accompanied by the estimate of peak power over the entire billing period, $\PrdPeak(T_0)$, based on the full sequence of daily chains across a month. This peak is generated by solving a MILP program that gives all the monthly chains as an input, and during training, this ``optimal peak'' across the month is used as an input for a given daily chain \ad{the whole concept of daily and monthly chains is a bit confusing and has to be cleared up. Basically how we reduce the monthly problem into a sequence of daily problems has to be described here clearly.}.


% Given the complexity of modeling state transition probabilities in the V2B problem, we conduct simulations for each billing period, referred to as a ``sample''. The simulator includes:
% \begin{itemize}[leftmargin=*] 
%     \item {The estimated peak power over entire billing period, $\PrdPeak(T_0)$ based on training samples.}
%     \item Electricity prices, $\theta_E(T_j)$ for $T_j \in \mathcal{T}$.
%     \item Building load, ${B}(T_j)$ for $T_j \in \mathcal{T}$.
%     \item EV arrival and departure schedules with SoC requirements, $\forall V \in \mathcal{V}: \SOCI, \SOCR, SOC, CAP$.
%     \item Available chargers and charging limits $\{C_i \in \mathcal{C}\}$.
% \end{itemize} 
The simulator updates the status of the building and chargers based on actions taken at each time slot. 
%The state transition function is defined as ${\it Trans}: \mathcal{S} \times \mathcal{A} \leftarrow \mathcal{S}$, with $(S(T_j), A(T_j)) \mapsto S(T_{j+1})$,  
%\rishav{change \\this and simulator\\ steps to use \\ ${T_j}$ \&$T_{j-1}$} 
%indicating how state features are updated.
This process includes the following steps: 

\begin{enumerate}[leftmargin=*]
    \item Initialize the estimated peak power, $\PrdPeak(T_0)$, which can be derived from historical data \ad{does not make sense. We need to clearly describe the process of how this is estimated for training as well as inference. Please update. There is no mention in section 4.2} (detailed in Section~\ref{ssec:pipeline}),
    , and update it by
    $
    \PrdPeak(T_{j+1}) = \max(\PrdPeak(T_j)$, $ \Building(T_j) + \sum_{C^i \in \mathcal{C}} P(C_i, T_j)),
    $
    which updates the estimated peak power depending on the previous estimate and the current peak power.
    \item Update SoC of EVs connected to all chargers: $\SOC(\phi(C_i,T_j), T_{j+1})$ using action $A(T_j)$ according to Equation~(\ref{eq: soc}). 
    %Additionally, we apply action post-processing to keep EV SoCs within valid boundaries by adjusting the power rate for stopping charging or discharging when they exceed $SoC^{\text{max}}(\phi(C_i, T_j))$ or drop below $SoC^{\text{min}}(\phi(C_i, T_j))$. 
   \item Update the EV charger assignment $\phi(C_i, T_j)$ and $\eta(V_k)$ by first releasing chargers with departing EVs in the next time slot $T_{j+1}$ and then assigning new arrival EVs to idle chargers, following the FIFO procedure and prioritizing the bi-directional chargers first. 
   \item Update the energy requirement of all EVs connected to a charger: $[\PowerNeed(C_i, T_{j+1})]_{C_i \in \mathcal{C}}$ (by Equation~(\ref{eq:chargerstate})) based on EV's current SoCs.
   \item Update the remaining time of all EVs connected to chargers: $[\ReTime(C_i, T_{j+1})]_{C_i \in \mathcal{C}}$ at time slot $T_{j+1}$.   
\end{enumerate}


{\bf Action Reward.} We define the function ${\it Reward}: \mathcal{S} \times \mathcal{A} \rightarrow \Re$, where ${\it Reward}(S(T_j), A(T_j))$ evaluates the reward for actions taken in a specific state, focusing on minimizing the total bill while satisfying SoC requirements. This function is expressed by: \ad{is the subscript index for actions is correct? }
\begin{align}
   & \mathit{Reward}(S(T_j), A(T_j)) = \lambda_{S} \cdot \mathit{Reward}_1 + \lambda_{E} \cdot \mathit{Reward}_2 + \lambda_{D} \cdot \mathit{Reward}_3
\end{align}
where, 
\begin{align*}
\begin{aligned}
    \mathit{Reward}_1 &=  \sum\limits_{C^i\in\mathcal{C}} \max(0, \min(\PowerNeed(C_i, T_j), P(C_i, T_j) \cdot \delta)) \\
    \mathit{Reward}_2 &= - P(C_i, T_j) \cdot \delta  \cdot \theta_E(T_j) \\
    \mathit{Reward}_3 &= - \max(0, \Building(T_j) + \sum\limits_{C^i \in \mathcal{C}} P(C_i, T_j) - \PrdPeak(T_j)) \cdot \theta_D
\end{aligned}
\end{align*}
% \begin{align}
%    & \mathit{Reward}(S(T_j), A(T_j)) = \nonumber \\
%    & \sum\limits_{C^i\in\mathcal{C}} \max(0, \min(\PowerNeed(C_i, T_j), P(C_i, T_j) \times\delta)) \times \lambda_{S} \nonumber \\
%    & - P(C_i, T_j) \times\delta  \times \theta_E(T_j) \times \lambda_{E} \nonumber \\
%    & - \max(0, \Building(T_j) + \sum\limits_{C^i \in \mathcal{C}} P(C_i, T_j) - \PrdPeak(T_j)) \times \theta_D \times \lambda_{D} 
% \end{align}
where $\mathit{Reward}_1$ promotes actions that charge EVs to reach their required SoC, as outlined in Eq. (\ref{eq: soc}). $\mathit{Reward}_2$ penalizes the energy costs generated by this action, and $\mathit{Reward}_3$ penalizes the increase in demand charges caused by rising peak power, aligning with our objective in Eq. (\ref{eq: billing}). These functions use three reward coefficients, $\lambda_{S}$, $\lambda_{E}$, and $\lambda_{D}$ to balance trade-offs between these reward factors. 
%The coefficients are adjustable during training to optimize model performance. 

% {\bf Policy}: Our objective is to develop the policy $\pi: \mathcal{S} \rightarrow \mathcal{A}$, where $\pi(S(T_j))$ generates the optimal charging actions for a given state, maximizing the overall action reward function throughout the billing period $T_j \in \mathcal{T}$.
 
% \rishav{Add discount factor \\short description}

==> sections/04_approach.tex <==
\section{Approach}
\label{sec:approach} 



% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}[b]{0.68\linewidth}
%         % \centering
%         \includegraphics[height=2.2in,keepaspectratio,trim=0.2cm 0.2cm 0.2cm 0.2cm,clip]{figures/framework.pdf}
%         % \vspace{-0.1in}
%         \caption{Reinforcement Learning Framework.}
%        \label{fig:framework}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}[b]{0.28\linewidth}
%         % \centering
%         \includegraphics[height=2.2in,keepaspectratio,trim=0cm 0.5cm 0cm 0.5cm,clip]{figures/inference_pipeline.pdf}
%         \vspace{-0.15in}
%         \caption{Pipeline for Inference.}
%         \label{fig:pipeline}
%     \end{subfigure}
%     \caption{\color{black}(a) Our framework relies on daily samples along with an estimated monthly peak power. A reinforcement learning policy based on DDPG is trained with policy guidance and action masking. These techniques improve the performance of the model. Finally, it generates charger actions for every given state. (b) At inference time $T_j$, the model requires data of connected cars, charger states and building load reading. It then uses a monthly peak power estimator to forecast the peak power for the entire billing period. The result are the charger actions for time $T_{j+1}$.}
%     \label{fig:framework_and_pipeline}
% \end{figure*}

% \begin{figure*}[t]
% \centering
% % \includegraphics[width=0.95\textwidth]{figures/framework_only.pdf}
% \includegraphics[width=0.95\textwidth]{figures/framework_v2.pdf}
% \caption{(Left) Data Processing Pipeline, (right) Complete Framework of our RLApproach.}
% \label{fig:framework_and_pipeline}
% \Description{}{}
% \end{figure*}


%We employ the Deep Deterministic Policy Gradient (DDPG) algorithm~\cite{lillicrap2015continuous} to train the policy $\pi(S(T_j))$ for the V2B problem. DDPG is ideal for handling our continuous action space and supports off-policy training, allowing the RL model to learn from diverse experiences across various scenarios, thereby enhancing model generalization. To enhance the policy performance, we propose integrating action masking and policy guidance techniques alongside DDPG, as outlined below. Figure~\ref{fig:framework_and_pipeline}.  

%. This framework enables optimal decision-making regarding charger power rates and load management, allowing for effective responses to uncertainties in user behaviors and building loads in our working scenario. We aim to derive a policy for each time slot that minimizes total costs while ensuring that the SoC requirements of the EVs are met throughout the billing period. 

%Considering the uncertainty in the V2B problem, we model it as a sequential decision-making problem using a Markov Decision Process (MDP) to simulate state transitions and utilize an RL-based approach to train a policy for this MDP. 

In this section, we first outline the data pipeline, focusing on how we handle the monthly training data, generate input features, and execute the policy (Figure~\ref{fig:framework_and_pipeline}) and then detail the MDP formulation. \ad{while the figure talks about delayed update, its discussion clearly in a highlighted paragraph is missing. This is an important part and hence must be emphasized.}
%, then discuss the steps of the data processing pipeline, 
 

\subsection{Data Pipeline}
\label{ssec:pipeline}
%To generate training and testing data for the RL models in the V2B problem, we follow these steps for data collection and processing. 
% % \begin{enumerate}[leftmargin=*] 
% \textbf{Data Collection}: We gather data from \nissan{}'s EV fleet, including arrival and departure times, initial SoC, and required SoC. We also collect historical smart building load demand across different seasons from May 2023 to January 2024. Additionally, data from EV chargers is collected, including charging/discharging rates.
    
% \textbf{Modeling for User Behavior and Building Load Fluctuation}: Based on the collected data, we model multiple features. For instance, we use the Poisson distribution to model EV arrivals at each hour, considering inputs such as current time, month, and weather information. Similarly, we train models using random forest to generate estimateed EV stay duration, initial SoC, and required SoC, effectively modeling EV driver behaviors. To model the building load fluctuation, we utilize 9 months of real building energy consumption data collected from \nissan{}'s smart building, recorded at 15-minute intervals. The building load is modeled using a normal distribution, with the real building load as the mean and introducing a standard error of 2 kW.

% \textbf{Generating Sample Chains for Training and Testing}: We then generate training samples for one-month billing period episodes, including EV arrival/departure schedules along with their initial SoC and required SoC, using the developed models for user behaviors. Building load data is generated at every 15-minute interval over a month. Additionally, we incorporate data for 15 \nissan{} EV chargers, consisting of 5 bidirectional and 10 unidirectional chargers. Time-of-Use (ToU) electricity rate schedules and demand charge data from utility providers are also integrated to simulate realistic billing scenarios. We generate 110 samples for each month from May 2023 to January 2025. Each sample contains all the above information for each day of the month, and we use 60 samples for training and 50 for testing.  
{\color{black} 
We outline the data pipeline in Figure~\ref{fig:framework_and_pipeline}, which encompasses the preliminary processes for RL training, detailing data collection, sample generation, peak power estimation, and training episode segmentation. \ad{clarify how much data exists. Also, clarify how we reduce the monthly problem to daily problem}
% These are all essential steps for effective RL training. 
 %  \textbf{Data Collection.} We first gather comprehensive data from \nissan{}'s EV fleet, including arrival and departure times, initial and required State of Charge (SoC), as well as historical smart building load demand across seasons from May 2023 to January 2024. Additionally, we collect charging and discharging rates from EV chargers. Multiple features are modeled to capture these distributions using the Poisson distribution for EV arrivals, SoC requirements, and building fluctuations based on historical data.

% \textbf{Generating Sample Chains for Training and Testing}. We create training samples for one-month billing episodes that encompass EV schedules, initial SoC, and required SoC. Building load flows are generated at 15-minute intervals based on historical data. We also integrate Time-of-Use (ToU) electricity rate schedules and demand charge data from utility providers to simulate realistic billing scenarios. 
% , as well as historical smart building load demand across seasons from May 2023 to January 2024. 
% Additionally, we collect telemetry data from EVs and EV chargers.
{\bf Sample generation.}
Data was collected and provided by \nissan{} from their fleet and chargers at their office building over the period from May 2023 to January 2024. The dataset includes EV arrival and departure times and initial and required State of Charge (SoC) as well as building power demand readings at 15 minute intervals. Since the location is categorized as an industrial building, it is subject to time-of-use (TOU) electricity rates and demand charges. TOU introduces variations in the electricity rates, with higher prices during peak hours (6:00 AM to 10:00 PM). Demand charge adds a flat rate multiplier to the highest average power delivery across 15-minute intervals over the billing period, and is added to the total bill.
To capture the distributions of these features, we utilize the Poisson distribution for modeling EV arrivals, SoC requirements, and building fluctuations based on historical data. We then empirically sampled $1000$ one-month billing episodes samples for each month from May 2023 to January 2024.  
% The building did not have data before May 2023 and data collection stopped in Jan 2024.

%Additionally, we integrate Time-of-Use (ToU) electricity rate schedules and demand charge data from utility providers to simulate realistic billing scenarios. Using these data models, we generate 1,000 samples for each month from May 2023 to January 2024. 

\textbf{Splitting data into daily episodes.}
\jpt{Can we explain a bit more on how splitting monthly to daily help with the training?}
To enhance training efficacy, we address the challenge of lengthy state-action episodes by splitting the monthly training dataset into daily episodes.
We focus only on weekdays since employees are often not present at the office, resulting in minimal EV arrivals and low building loads, both of which do not significantly impact the overall monthly demand charge. We incorporate the estimated monthly peak power as an input feature and penalize only those peak power values exceeding this estimated value in each daily episode. This approach incentivizes the policy to minimize the monthly peak power while effectively training with daily episodes.

{{\bf Down-sampling Strategy}.
During training, we varied the amount of samples used for training and observed that utilizing a larger number of training episodes results in longer convergence time and overall worse performance. We show the results of this in~\Cref{ssec:ablation}.
% During training, we implement a down-sampling strategy from the 1,000 monthly samples. We observe that utilizing the complete dataset results in excessive training iterations, significantly increasing the training duration (up to 3 days on our computing systems) and complicating convergence, motivating us to perform down-sampling. 
Thus, we utilize a k-means clustering approach to down-sample. We used $k=5$ and clustered using the optimal demand charge derived from the MILP solution for each sample. 
% This optimal demand charge is closely correlated with sample characteristics, such as building load distribution and EV user's behavior, and significantly influences the total bill. 
% Specifically, We clustered 1,000 samples into five groups based on optimal demand charge using k-means. 
From each cluster, we select 60 and 50 samples for the final training and testing datasets respectively, ensuring that these datasets are mutually exclusive. 
% This method allows us to train and evaluate our RL model using fewer but representative training samples, thereby mitigating the loss of diversity and distribution among the samples.
}

\textbf{Peak power estimation.} 
% A key aspect of our state definition is the monthly peak power estimation. 
We employ a MILP solver to determine the minimum demand charge derived from optimal action sequences over the one-month billing period across all training samples. From the distribution of peak power from the MILP solutions, we set the lower bound of the 95\% confidence interval as the estimated peak power for the month, providing a conservative initial estimate.



%{\bf Data Collection}: We gather data from \nissan{}'s EV fleet, including arrival and departure times, initial and required State of Charge (SoC). Historical smart building load demand is collected across seasons from May 2023 to January 2024, along with charging and discharging rates from EV chargers. Multiple features are modeled to capture these distributions, employing the Poisson distribution for EV arrivals, SoC requirements, and building fluctuations based on historical data.
%{\bf Generating Sample Chains for Training and Testing}: We create training samples for one-month billing episodes, encompassing EV schedules, initial SoC, and required SoC, using the developed models. Building load flows are generated at 15-minute intervals based on historical data. Additionally, Time-of-Use (ToU) electricity rate schedules and demand charge data from utility providers are integrated to simulate realistic billing scenarios.

% \textbf{Feature Generation}: Based on the cleaned data, we generate input features such as building load profiles, EV arrival schedules, initial SoC, and departure SoC targets. These features serve as the input states for the RL model training and testing phases. 
% This process ensures that the RL models are trained on accurate and diverse data, providing robustness and generalization across various V2B scenarios.

%{\bf Generating samples.} To assess our RL-based V2B charging optimization approach, we used real-world data collected {\color{black} from an \nissan{}'s office building, along with charger meter readings in Santa Clara, California.} This data was used to derive statistics and develop generative models for generating samples for training and testing the RL model, which also serves as input to our simulator.

%\textbf{Monthly Peak Power estimation:} Our state definition includes an initial peak power estimation over the whole billing period as an input feature. We employ a Mixed-Integer Linear Programming (MILP) solver to determine the minimum demand charge derived from optimal action sequences over a one-month period across all training samples. For each month, we analyze the distribution of peak power from the MILP solutions and use the lower bound of the 95\% confidence interval as the estimated monthly demand charge, providing a conservative initial estimate. 
 
%{\bf Splitting Training Data into Daily Episodes:} During our training process, we encountered a challenge: utilizing a one-month billing period resulted in lengthy state-action episodes, hindering the policy's ability to learn the Q-value effectively. To address this, we reduced the training episodes to daily segments, focusing on weekdays. This decision was informed by our observation that weekends often have infrequent EV arrivals and low buidling load, which do not significantly impact the overall monthly demand charge.  To ensure that monthly peak power considerations are integrated, we incorporate the estimated monthly demand charge as an input feature. Additionally, the reward function penalizes only those demand charges that exceed this estimated value in each daily episode. This approach incentivizes the policy to minimize the monthly demand charge while effectively training with daily episodes.

{\bf Model inference.} Our RL-based policy operates at $delta$ intervals to determine current policy actions. To generate these actions, we require a set of input data, including the charger status (connected EV's current SoC, expected departure time, current building load, and charger information), the charging rate limits for each charger, and the estimated peak power. 
%{which can be derived from historical data or machine learning-based predictive models}.
In this paper, we utilize the estimated peak power based on training samples. With this current information, we abstract the input features for the RL model, enabling it to determine the power rate control actions for the upcoming time interval.
} 



\subsection{Environment Simulator}
Our approach uses stateless discrete event simulator that serves as the digital twin of our target environment. It holds a state that represents the entirety of the world. This includes information on EVs, building, and the grid. This allows us to investigate how any action or decision can potentially impact the real world. Decisions are taken at the end of each set of events for any given time period. There are two main decisions that must be taken when solving the V2B charging problem. (1) Charger assignments and (2) Charger actions. We address the charger assignment decision below and provide information on the charger action in~\Cref{sec:RL}.

\textbf{Environment updates.} The input episodes serve as the entirety of the simulator's world view. Each event includes an event type and time, matching their real world trigger and occurrence. We identify several critical events in the episodes to serve as the triggers for the simulator. These include (1) EV arrivals, (2) EV departures, (3) building power readings, and (4) TOU rate changes. Events are placed in a queue, with each event triggering an update to the environment which modifies the state. Updates to the state, which include the charging or discharging of EVs, are based on the elapsed time between events. Only EV arrival events trigger charger assignment decisions, while all events trigger a charger action decision.

\input{results/charger_assignments}
\textbf{Charger assignment.} In our approach we consider a first-in, first-out policy that prioritizes the assignment of EVs to bidirectional chargers. If multiple EVs arrive at the same time, then we break the ties randomly. \Cref{table:charger_assignment_policies} shows the different charger assignment and tie breaking policies tested. Bidirectional charging assignments outperform any other assignment policy. Tie breaking policies that favor latest departing cars have marginal advantage over others. While the assignment policies can be further optimized, we elected to follow this heuristic, focusing instead on the second decision problem of charger action.

\textbf{Charger actions.} We provide several policies with our simulator to contrast and compare with our proposed approach. Charger action policies receive a state of the environment for a particular time and generate actions based on this. The simulator is stateless. Thus, it provides only a current representation of the world at that specific time to each policy.


\input{sections/02_2_MDP}


==> sections/04b_ReinforcementLearning.tex <==
% \begin{algorithm}[t]
% \setcounter{AlgoLine}{0} %
% \small
%     \SetAlgoLined
%     \KwIn{Initial policy parameters for actor network $\zeta_a$, critic parameters $\zeta_c$, target network parameters $\zeta_a', \zeta_c'$\\
% Training parameters: $\mathit{actionNoise}$, $\policyGuidanceRate$, $\mathit{bufferSize}$, $\mathit{batchSize}$, maximum training iterations: $M$}
%     \KwOut{Trained policy $\pi_{\alpha}$}
%     Initialize replay buffer $\Buffer$ \\
%     % Initialize target network weights $\zeta_a' \leftarrow \zeta_a$, $\zeta_c' \leftarrow \zeta_c$ \\
%     \For{$1$ \KwTo $M$}{
%         $s_0$ \gets initial state from the simulator 
%         % Initialize a random process $N$ for action exploration 
        
%         \For{each time slot $T_j \in \mathcal{T}$}{
%         % \If{$T_j$ is during non-peak hours}{
%         % Get action A(T_j) using h
%         %}
%         \tcp{Introducing policy guidance stochastically.}
%             {\color{black} randomValue $\leftarrow randomBetween(0,1) $
            
%             \If
%             %(\tcp*[h]{Adding policy guidance stochastically}) $$
%             { randomValue $\leq \policyGuidanceRate$}{
%         Get action $A(T_j)$ by rerunning the ILP solver: $A(T_j)\leftarrow\MILP(S(T_j), {\it remainEpisode})$
%                 }
%             \Else{
%                 % $A(T_j)\gets  \pi(S(T_j) | \zeta_a) + \mathit{actionNoise}$
%                 Get masked action $A(T_j) \gets \Mask\left(S(T_j), \pi(S(T_j) | \zeta_a)) + \mathit{actionNoise} \right)$ by current policy and $\mathit{actionNoise}$  
%                 % \tcp{Add action masking}
%             }}
%              State transition $S(T_{j+1})\leftarrow {\it Trans}(S(T_j), A(T_j))$. 
%             %in Algorithm~\ref{alg: stateTrans}. 

%             Get the action reward $R(T_j)\leftarrow {\it Reward}(S(T_j), A(T_j))$. 
%             %by Algorithm~\ref{alg: reward}. 
            
%             Store transition $(S(T_j), A(T_j), R(T_j), S(T_{j+1}))$ in $\Buffer$

%             Sample a minibatch $(S(T_i), A(T_i), R(T_i), S(T_{j+1})$ from $\Buffer$ 

%            {\color{black} Get masked actions $A(T_{i+1})$ at $S(T_{i+1})$ using target actor network: $A(T_{i+1})\leftarrow \Mask(S(T_{i+1}), \pi'(S(T_{i+1}) | \zeta_a'))$}  
%             %using Algorithm~\ref{alg: mask}  \tcp{Add action masking}

%             Set target $y_i\leftarrow R(T_j) + \gamma Q'(S(T_{i+1}), A(T_{i+1})
%             | \zeta_c')$ 
            
%             Update critic network by minimizing the loss: $L 
%             \leftarrow \frac{1}{N} \sum_i (y_i - Q(S(T_i), A(T_i) | \zeta_c))^2$ 
            
%              {\color{black} Get masked actions $A(T_i)$ at $S(T_i)$ using actor network: $A(T_i)\leftarrow \Mask( S(T_i), \pi(S(T_i) | \zeta_a))$ }%using Algorithm~\ref{alg: mask}.  
%              % \tcp{Add action masking}
%            % Mask action $A(T_i)\leftarrow \Mask(S(T_i), a_{i})$ 
           
%             Update the actor policy by policy gradient: 
%             $\nabla_{\zeta_a} J \leftarrow \frac{1}{N} \sum_i \nabla_a Q(S(T_i), A(T_i) | \zeta_c) | \nabla_{\zeta_a} \pi(s | \zeta_a) |_{S(T_i)}$
            
%             Delayed Update the target networks: 
%             $\zeta_a' \leftarrow \tau \zeta_a + (1 - \tau) \zeta_a'$; 
%             $\zeta_c' \leftarrow \tau \zeta_c + (1 - \tau) \zeta_c'$ \\
%         }
%     }
%     \caption{Improved DDPG with Action Masking and Policy Guidance.}
% \label{alg:DDPG} 
% \end{algorithm}

%%%%%%%%%%%% ACTION MASKING %%%%%%%%%%%%
\begin{algorithm}[ht]
    \SetAlgoNlRelativeSize{-1}
    \KwIn{$\textit{state}, \textit{action: } A(T_j) $}
    \KwOut{Masked action: $\MaskAction$} 
\small
$\PowerNeed \gets [\PowerNeed(C_i, T_j)]_{C_i \in \mathbf{C}};$
$\ReTime \gets [\ReTime(\phi(C_i, T_j))]_{C_i \in \mathbf{C}};$
$\epsilon \gets 10^{-5};$
$C^{max} \gets [C^{max}_i]_{C_i \in \mathbf{C}};$
$C^{min} \gets [C^{min}_i]_{C_i \in \mathbf{C}};$

\tcp{Mask 1: Set action = 0 if no car is connected}
    $ \MaskAction \gets \frac{\ReTime}{\ReTime + \epsilon} \times A(T_j)$\;
    
    \tcp{Mask 2: Stop charging when required SoC is reached for uni-directional chargers}
    $ \MaskAction_{tmp} \gets \MaskAction$; 
    $\MaskAction_{tmp} \gets \min(\MaskAction_{tmp}, \frac{\PowerNeed}{\delta})$\;
    $ \MaskAction[\textit{uniIdx}] \gets \MaskAction_{tmp}[\textit{uniIdx}]$\;

    \tcp{Mask 3: Enforce charging to the required SoC before departure. }
    $\overline{\Power(T_j)} \gets \frac{ \PowerNeed- (\ReTime - 1) \times C^{max} \times \delta }{\delta}$\;
    $\overline{\Power(T_j)} \gets \min(\overline{\Power(T_j)}, C^{max})$\;
    $ \MaskAction \gets \max(\MaskAction, \overline{\Power(T_j)})$\;
    \tcp{Mask 4: Ensure bidirectional chargers discharge to the required SoC before departure.}
    $\Power^*(T_j) \gets \frac{\PowerNeed- (\ReTime - 1) \times P_{min} \times \delta }{\delta}$\;
    $\Power^*(T_j) \gets \max(\Power^*_t, P_{min})$\;
    
    $\MaskAction_{tmp}\gets \MaskAction$; 
    $ \MaskAction[\textit{biIdx}] \gets \min(\MaskAction_{tmp}, \Power^*_t)[\textit{biIdx}]$\;

    \tcp{Mask 5: Power improvement strategy}
    $ \textit{powerGap} \gets \Building(T_j) - \PrdPeak(T_j)$\;
    $ \textit{canIncrease} \gets \textit{RELU}\left(\max\left(\frac{\PowerNeed}{\delta}, C^{max}\right) - \MaskAction \right)$\;
    
    $ \textit{toImprove} \gets \min\left(\textit{RELU}(\textit{powerGap} - \sum \MaskAction), \sum \textit{canIncrease}\right)$
    
    $ \MaskAction \gets \MaskAction + \frac{\textit{toImprove} \times \textit{canIncrease}}{\sum(\textit{canIncrease}) + \epsilon}$\;

    \tcp{Mask 6: Do not discharge below building load}
    $ \textit{toImprove} \gets \max(-\Building(T_j) - \sum(\MaskAction), 0)$\;
    $ \textit{negAction} \gets \textit{RELU}(\MaskAction \times -1) \times -1$\;
    
    % $ \textit{toIncrease} \gets \frac{\textit{toImprove} \times \textit{tmpAction}}{\sum(\textit{tmpAction}) + \epsilon}$\;
    $ \MaskAction \gets \MaskAction +  \frac{\textit{toImprove} \times \textit{negAction}}{\sum(\textit{negAction}) + \epsilon}$\;

    \caption{Action Masking: $\Mask(S(T_j), A(T_j))$.} 
    \label{alg: action_masking}
\end{algorithm} 

% Based on the formulated MDP, we next use a RL approach to train a policy that maximizes long-term rewards by interacting with a custom environment simulator, which processes all data samples and handles state transitions.  
% \subsection{Environment Simulator}
% \jpnote{I will add this, just talk about how the transition is represented by the simulator. See Mike's paper.}



\section{Reinforcement Learning Policy}
\label{sec:RL}
% Figure~\ref{fig:framework_and_pipeline}. We input the the training data into our designed environment simulator, which handle the state generation and state transformations based on actions following our state transition function described in Section~\ref{ssec:MDP}.

% Based on the formulated MDP, we discuss the RL-based framework used for policy training to maximize the long-term reward of this MDP, as shown in \Cref{fig:framework}. This paper utilizes the Deep Deterministic Policy Gradient (DDPG) algorithm~\cite{lillicrap2015continuous} for policy training. DDPG is well-suited for handling continuous action spaces and supports off-policy training, enabling the model to learn from diverse experiences across various scenarios, thus improving generalization. 

% To further enhance policy performance, we integrate action masking and policy guidance techniques with DDPG. An overview of the RL-based framework shows that we input the training data into our designed environment simulator, which generates state transitions and transformations based on actions according to the state transition function described in Section~\ref{ssec:MDP}. In traditional DDPG, the actor network generates state and action trajectories through interaction with the environmental simulator, which are then stored in the replay buffer for training the critic and actor networks.  
% In this work, we enhance this process with a policy guidance approach. Instead of solely relying on the actor network for training trajectories, we incorporate a MILP solver to provide optimal actions based on current and future information, guiding the RL training away from local optima. Additionally, we implement an action masking procedure, represented as $\Mask(S(T_j), A(T_j))$, which refines the raw actions from the actor network by considering constraints for action validity and utilizing domain-specific knowledge to limit the exploration range of training actions and improve policy performance.  
% Our advanced DDPG method is described as follows. Algorithm~\ref{alg:DDPG} depicts our customized DDPG approach, incorporating action masking and policy guidance. This approach builds upon the classic DDPG algorithm by introducing policy guidance (lines 5 to 9) and action masking (lines 9, 14, and 17).
%Based on the formulated MDP, we present an RL-based framework for policy training aimed at maximizing long-term rewards, as illustrated in \Cref{fig:framework}. 
During training, data samples are input into our designed environment simulator \ad{as mentioned before we do not describe simulator enough, perhaps more information and statement that we will cite the simulator after blind review}, which provides the environment that abstracts state features for the RL models and manages state transitions based on the function described in Section~\ref{ssec:MDP}. The simulator operates based on actions (power rates) generated by the policies and dynamic events such as EV arrivals and departures. 
Our core approach is based on  Deep Deterministic Policy Gradient (DDPG) algorithm~\cite{lillicrap2015continuous}, which  is well-suited for continuous action spaces and supports off-policy training, allowing the model to learn from diverse experiences across various scenarios, thereby improving generalization. To enhance the policy performance, we integrate action masking and policy guidance techniques with DDPG as outlined in Algorithm~\ref{alg:DDPG}.  

Traditional DDPG relies on the actor network to generate actions (power rates in this work). The tuples of state, action, action reward, and next state are stored as state transitions in the replay buffer (see lines 9 to 12). In each training iteration, we batch state transitions from the replay buffer for model training (see line 13). Specifically, DDPG maintains target networks for both the actor and critic, which are used to generate the next state and compute Q-values essential for calculating the critic loss during training. The critic network is trained using gradient descent by minimizing the mean squared error between predicted Q-values and target Q-values derived from the Bellman equation (see lines 14 to 16). The critic learns Q-values for state-action pairs, which are then used to train the actor network through a policy gradient approach (see lines 17 and 18). These target networks are updated less frequently to stabilize the training process (see lines 18 and 19). 

To address the large state and action spaces in this RL model, we enhance DDPG by integrating an action masking procedure, denoted as $\Mask(S(T_j), A(T_j))$. This procedure refines the raw actions generated by the actor network by enforcing action validity and utilizing domain-specific knowledge, thereby improving policy performance. The action masking is applied after the actor network produces raw actions, acting as an additional layer (see lines 9, 14, 17). 
Additionally, we implement a policy guidance procedure (see lines 5 to 9) by incorporating a MILP solver to provide optimal actions through the function $\MILP(S(T_j), {\it remainEpisode})$, based on current and future information. These optimal actions are stochastically introduced during RL training into the replay buffer, mixing high-quality actions with the raw RL actions to enhance the training transition quality and guide the RL training in a beneficial direction. 

Next, we detail our RL framework by outlining the design of the environment simulator, the data normalization and network structure, the action masking and policy guidance procedures, and the heuristic approaches used to simplify our RL training. 
%which incorporates both policy guidance (lines 5 to 9) and action masking (lines 9, 14, and 17). 


% During training, optimal actions are stochastically incorporated into the process based on a predefined ratio coefficient, denoted as $\policyGuidanceRate$, and stored in the replay buffer. The function $\MILP(S(T_j), {\it remainEpisode})$ takes the current state as input and outputs the next optimal action. It can also access remaining events in the episode, including upcoming EV arrivals, SoC requirements, and building load, to invoke a MILP solver. This solver generates a sequence of optimal actions starting at timestamp $t$, returning the first action in the sequence, which serves as the optimal action for the current state to maximize long-term reward (lines 5 to 9).



\subsection{Actor-Critic Network Structure} 
%\jpnote{Add sentence description of the number of layers we are considering for the Actor Critic models}
To enhance convergence and improve generalization, we preprocess all state variables to be within the range of 0 and 1 before feeding them into neural networks. Timestamps are normalized by dividing the number of minutes in a day, while power-related variables such as building load $\Building(T_j)$, estimated peak power $\PrdPeak(T_j)$ are scaled by their respective statistical factors. Furthermore, we normalize the energy capacity $CAP(V_k)$ of each car by dividing it by the maximum capacity among EVs. 
For the action $A(T_j)=[P(C_i, T_j)]_{C^{i}\in \mathcal{C}}$. We normalize the action values to the range of $[-1, 1]$ based on the power rate range $[C_i^{min}, C_i^{max}]$ by Equation~(\ref{eq: normalize}).
\begin{equation}
    \hat{P}(C_i, T_j)=\frac{2\times(P(C_i, T_j)-C_i^{min})}{C_i^{max} - C_i^{min}}-1. 
\label{eq: normalize}
\end{equation}
% In DDPG, two neural networks are employed: the critic network evaluates state Q-values, while the actor network generates deterministic actions as the policy.
% The critic network processes state and action inputs through hidden layers (2 layers used in final model) with ReLU activation, outputting a single Q-value estimate.
Both critic and actor network have two hidden layers with 96 neurons each. Both feature a ReLU activation layer at the end. The critic network outputs a single Q-value estimate while the actor network outputs the action which represent the power rate of each charger.
% The exact size used in the model are described in~\Cref{tab:hyperparameters}.
% Simultaneously, the actor network maps the input state through multiple hidden layers (2 layers used in final model) with ReLU activations to produce the action output, representing the power rate of each charger.
This output is constrained within the range $[-1, 1]$ using a $\tanh$ activation function. The original charging power values can be obtained by computing the inverse of the normalization equation in Equation~(\ref{eq: normalize}).  \ad{this section needs clear revision. It should just tell how the network is structured and how data is normalized and input into the network. Also, clear description of the size and architecture is required.}
\jpt{I modified the text, it still needs the normalization part.}



\subsection{Action Masking}
\label{sec: DDPG} 

%\jpnote{Move the algorithm ahead of this and summarize your points while referring to the algorithm. You can add label commands to the lines of the algorithm to refer to it. Also rename your heuristic and constraints in the algorithm to just action masking N}

We propose action masking approach addresses the challenge of large continuous action spaces (detailed in Algorithm~\ref{alg: action_masking}), by ensuring that the policy actions generated by the actor network are valid and reasonable during DDPG training. This technique, based on findings from \cite{huang2020closer,kanervisto2020action}, confirms that differentiable action masking does not interfere with the policy gradient backpropagation process. As a result, the learning process remains effective, while the imposed constraints on the action space prevent the actor network from exploring invalid actions, thereby improving training efficiency and optimizing resource usage.

This procedure takes the RL raw action $A(T_j)$, an array of power rates $[P(C_i, T_j)]_{C_i\in\mathcal{C}}$ for all chargers, processes it through the following steps, and outputs the masked actions $A'$. Before computing, we first obtain the state features formatted as arrays: the remaining power needed to reach the required SoC for all connected EVs ($\PowerNeed$), their remaining time ($\ReTime$), and the maximum ($C^{\max}$) and minimum ($C^{\min}$) power rates of all chargers (see line 1). Also, we denote ${\it uniIdx}$ and ${\it biIdx}$ as the indices for unidirectional and bidirectional chargers, respectively.    
% \jpnote{Shorten the descriptions and make it very concise.} 
\begin{itemize}[leftmargin=*]
    \item \textbf{Mask 1.} 
    %We masks the action by setting the powe rate $P(C_i, T_j)$ of charger $C_i$ to 0 if no EV is plugged in. This method effectively masks all actions for idle chargers (where $\ReTime(\phi(C_i, T_j))=0$ indicates no EV is connected to charger $C_i$ at time slot $T_j$).
    We set the power rate $P(C_i, T_j)$ of charger $C_i$ to 0 if no EV is plugged in, effectively masking actions for idle chargers (where $\ReTime(\phi(C_i, T_j))=0$).
    %%%
    \item \textbf{Mask 2.} Overcharging unidirectional chargers is unbeneficial since excess energy cannot be discharged. Thus we limit the power rates to ensure the SoC of unidirectional chargers remains within required SoCs. 
    %by masking the actions using the minimum of the current power rate and the rate required for EVs to reach the required SoC after this time slot, calculated as $\PowerNeed/\delta$. 
    Actions are masked to the minimum of the current power rate and the rate needed for EVs to reach required SoC, calculated as $\PowerNeed/\delta$ (see lines 3 and 4).
    % The rationale behind this approach is that overcharging unidirectional chargers offers no benefit, as the excess energy cannot be discharged 
    %%%
    \item \textbf{Mask 3.} 
    %Action are masked to minimize the missing SoC for all EVs at the time of departure, as outlined in objective function~(\ref{eq: soc_penalty}).
    Actions are adjusted to forced charging to required SoC before departure if necessary, to minimize missing SoC as per objective function~(\ref{eq: soc_penalty}).  
    We compute the critical power rate $\overline{\Power^*(T_j)}$, representing the minimum required power rate for all chargers at time $T_j$ to their required SoC before departing (assuming maximum power is subsequently utilized). The raw action is adjusted if it falls below this rate, especially in final time slots (see lines 5 to 7).
    %At each time slot, we compute the critical power rate $\overline{\Power^*(T_j)}$, which represents the minimum power rate required for all chargers at time $T_j$ to ensure that all connected EVs reach the required SoC before departing (assuming maximum power is subsequently utilized). The raw action is adjusted if it falls below this critical power rate. 
    
    \item \textbf{Mask 4.} 
    Overcharging bidirectional EVs is only advantageous if excess energy can be discharged during peak hours; thus, there’s no benefit to overcharging just before departure. Thus, we adjust actions to prevent discharging EVs if the raw action would cause exceeding the required SoC before departure.  Here, $\Power^*(T_j)$ denotes the minimum power rate needed for all chargers $C_i \in \mathcal{C}$ at time $T_j$ (see lines 8 to 10).
    %We mask action to discharge EVs to reduce their SoC if the raw action would result in exceeding the required SoC before departure. The intuition behind this is that overcharging EVs in bidirectional chargers is advantageous only when the excess energy can be discharged during peak hours to mitigate demand charges; thus, there is no benefit to overcharging them just before departure. Here, $\Power^*(T_j)$ denotes the minimum power rate required for all chargers $C_i \in \mathcal{C}$ at time $T_j$ to ensure that all EVs connected to bidirectional chargers can discharge to the required SoC before leaving (see lines 8 to 10). 
    
    %%%
    \item \textbf{Mask 5.} 
    %We mask action to increase charging power rates while ensuring that the masked action remains within the estimated peak power limit. The goal is to encourage charging to the required SoC without raising the demand charge, thereby avoiding forced charging just before departure, which could elevate peak power. In this step, we calculate the power gap between the estimated peak power and the current building load, represented as $\PrdPeak(T_j) - \Building(T_j)$. If the current sum of action power is below this gap, we utilize the available power gap to enhance the current action by allocating the additional power needed. This allocation is constrained by the maximum power rate each entity can increase and the power required to reach the required SoC of the connected EVs, computed using ${\it canIncrease}$ (see lines 11 to 14). 
    We increase charging power rates while ensuring the masked action stays within the estimated peak power limit. This aims to charge EVs to their required SoC without raising demand charges, thereby avoiding forced charging just before departure, which could elevate peak power. 
    We calculate the power gap between estimated peak power and current building load, $\PrdPeak(T_j) - \Building(T_j)$. If the current power sum is below this gap, we enhance the action using the available power gap, constrained by the maximum rate each EV can increase to reach the required SoC, computed using ${\it canIncrease}$ (see lines 11 to 14). 
    %constrained by the maximum power increase and the required SoC of connected EVs (see lines 11 to 14).
    
    %%%
    \item \textbf{Mask 6} We adjust the discharging power rate to prevent discharging below the current building load $\Building(T_j)$ by increasing negative actions based on their current values (see lines 15 to 17). 
\end{itemize} 

All above action masking procedures utilize array computations and differentiable operations, such as ReLU \cite{rasamoelina2020review} and maximum/minimum operations, from the PyTorch library \cite{paszke2017automatic}. 







 % We then employ \textbf{Heuristic 2}, which ensures that all EVs' charging needs are met by enforcing minimum power rates $P(C_i, T_j)$ when the remaining time is insufficient to reach the required SoC ${\it SoC}^{\text{req}}(v)$ using the maximum power rate.

% We then employ \textbf{Heuristic 2}, which ensures that all EVs reach their required SoC at departure. This is achieved by enforcing maximum power rates \( P(C_i, T_j) \) when the remaining time is insufficient to reach the required SoC $ {\it SoC}^{\text{req}}(v) $ using the maximum power rate. 
% This step ensures that all chargers charge the EVs to the required SoC before departure, if feasible. Additionally, this forced charging is applied only in the final time slots when it is required.

%We denote ${\it uniIdx}$ and ${\it biIdx}$ as the indices of the uni-directional and bi-directional chargers, respectively.   
%We introduce \textbf{Heuristic 3}, which bounds discharging to allow EVs to reduce their SoC if it exceeds the required levels. The intuition is that there is no benefit to overcharging in bidirectional chargers before departure.






\subsection{MILP Policy Guidance} 

To address the challenge of local optima in DDPG, we  integrate a policy guidance approach~\cite{pmlr-v28-levine13} into the RL training process. This aims to improve performance by providing optimal actions to guide the training toward better outcomes. We implement an optimization framework to generate optimal actions and add them to the replay buffer, providing effective guidance to steer the search towards global optima. Specifically, we formulate the V2B problem using mixed-integer linear programming (MILP). We give the MILP solver the current state information, including the current EV status, charge usage, and all future events from the input sample (EV arrival/departure, building load flow, and electricity prices from the current time to the end of the billing period. The MILP solution provides the power rate for each charger from the current time to the end of the billing period, maximizing the multi-objective weighted sum of total cost (detailed in Equation~(\ref{eq: billing})) and penalties for missing SoC requirements (defined in Equation~(\ref{eq: soc_penalty})). Following multiple constraints related to the EV SoC update  function following Equation~(\ref{eq: soc}) and Constraints~(\ref{eq:charging_rate}) to (\ref{eq:building_power}).   

% During training, optimal actions are stochastically incorporated into state transitions process based on a predefined ratio coefficient, denoted as $\policyGuidanceRate$, and stored in the replay buffer (as shown in Algorithm~\ref{alg: DDPG}. The function $\MILP(S(T_j), {\it remainEpisode})$ takes the current state as input and outputs the next optimal action. It can also access remaining events in the episode, including upcoming EV arrivals, SoC requirements, and building load, to invoke a MILP solver. This solver generates a sequence of optimal actions starting at timestamp $t$, returning the first action in the sequence, which serves as the optimal action for the current state to maximize long-term reward (lines 5 to 9). 
During training, optimal actions are stochastically incorporated into the state transition process based on a predefined coefficient, denoted as $\policyGuidanceRate$, and stored in the replay buffer (see Algorithm~\ref{alg:DDPG}). The function $\MILP(S(T_j), {\it remainEpisode})$ takes the current state as input and outputs the next optimal action. It considers remaining events in the episode, such as upcoming EV arrivals, SoC requirements, and building load, to invoke a MILP solver. This solver generates a sequence of optimal actions starting at time slot $T_j$ and returns the optimal action for the next time slot, serving to maximize the long-term reward. 

%SoC requirement,
% which ensure EVs must reach their required SoC before departure.
% \[
% SoC_{T_d(v)}(v) \geq So
% \]   
% Using the MILP solution, we can generate actions based on any state to maximize the long-term reward. 
% {\color{black} 
% The MILP aims to minimize the total energy cost, including both consumption and demand charges, while ensuring that all EVs meet their SoC requirements before departure. The objective function is:
% \[
% \min \Cost^{\it EN}(\mathcal{P}) + Cost^{\it DC}(\mathcal{P})
% \]
% as shown in Equations~\ref{eq: objective_1, eq: objective_2}. 
% where \( g_t \) represents the energy usage cost at time slot \( t \in \mathcal{T} \), \( P_{\text{max}} \) is the maximum power consumed during peak hours.  
% The model includes binary variables for charger assignments (\( a_{v,cp,s} \)), and continuous variables for charging rates (\( c^v_s \)) and battery levels (\( e^v_s \)). Key constraints ensure that: 
% \begin{enumerate}
% \item \textbf{Charger Assignments}: Each EV \( v \) is assigned to at most one charger \( cp \) at any time slot \( s \), and charger capacities are not exceeded, and is denoted by the assignment variable $a \in \mathcal{A}$.
% \[
%  \sum_{C_i \in \mathcal{C}} a_{v,i,s} \leq 1
% \]
        
% \item \textbf{SoC Requirements}: EVs must reach their required SoC before departure.
% \[
% SoC_{T_d(v)}(v) \geq SoC^(v)
% \]  
% \item \textbf{Energy Balance}: The energy in the EV battery evolves according to the charging rate, where $C_i$ is the charger attached to car $v$ indicated by Equation~(\ref{eq: SoC}). 
%     % \[
%     % SoC_{t+1}(v) = SoC_{t}(v) + P(C_i, T_j)
%     % \]
% \item \textbf{Demand Charges}: Demand charges are incorporated by modeling the maximum power consumption, as indicated by Equation~\eqref{eq: objective_2}.
% \end{enumerate}
% By solving this MILP using current state information and future events (e.g., EV arrivals/departures, building load, electricity prices), we generate optimal action sequences that maximize the long-term reward. These optimal actions are then stochastically introduced into the replay buffer during DDPG training, effectively guiding the RL agent towards global optima and improving training outcomes.
% } 
% The final DDPG approach, incorporating action masking and policy guidance, is depicted in Algorithm~\ref{alg: DDPG}. 
% {\color{black} This approach builds upon the classic DDPG algorithm by introducing policy guidance (lines 5 to 9) and action masking (lines 9, 14, and 17). 
 %This procedure ensures valid and efficient action selection, leading to improved training outcomes in DDPG. 
%The lines in {\color{black}black} highlight the enhancements over the classic DDPG. These colored the sections involve policy guidance and action masking. During DDPG training, optimal actions are stochastically introduced based on a predefined ratio coefficient $\policyGuidanceRate$ and stored in the replay buffer. We define the $\MILP(S(T_j))$ function to invoke the MILP solver and generate a sequential optimal action sequence starting at timestamp $t$, returning the first generated action which represents the optimal action for the current state (see lines 5 to 9). This procedure ensures both valid and efficient action selection, leading to improved training outcomes in DDPG.  


% {\color{red} Add text connecting two subsections. }
% \begin{itemize}[leftmargin=*]
%     \item {\bf Least Laxity First (LLF)}: Least Laxity First is a dynaimc priority driven algorithm designed for scheduling multiprocessor real time tasks~\cite{leung1989new}. Laxity or slack time refers to the amount of time a task can be delayed without causing it to miss its deadline. In the context of EV charging, we define laxity as the difference between the amount of time remaining for a car before it departs and the amont of time it takes to meet the user's required SoC at a constant rate of charge~\cite{xu2016dynamic}. Additionally, we limit the amount of cars charging at any given time interval by allocating a capacity at each step. The capacity is based on the difference between a set a power threshold and the current building load at that time. 
%     Only cars connected to chargers whose aggregate power rates fall within this limit are able to be charged for that time interval. LLF will provide trickle charge, charging the cars to the minimum required power to reach required SoC before departure, at each interval. 
% \end{itemize} 
\subsection{Heuristic Approach and Post Processing}
% \jpnote{Clarify what this section is, is this in the figure 2A?}
% We observe that off-peak hours typically feature lower electricity prices, allowing for charging EVs at a higher power rate without impacting the final demand charge. This insight leads us to maximize EV charging during off-peak hours, thereby reducing energy costs and alleviating pressure on charging during peak hours. To implement this strategy, we employ a greedy approach that directs the charging of all EVs to their required SoC at the maximum power rate. Additionally, discharging to the required SoC is performed when entering the off-peak duration after peak hours.
% We observe that off-peak hours typically offer lower electricity prices, enabling EV charging at a higher power rate without affecting the final demand charge. This insight allows us to maximize EV charging during off-peak hours, reducing energy costs and alleviating pressure on charging during peak periods. To implement this strategy, we adopt a greedy approach to manage off-peak charging, replacing the RL models. This approach directs the charging of all EVs until they reach their required SoC at the maximum power rate during off-peak hours. Additionally, discharging occurs when entering off-peak periods after peak hours if the current SoC of the EV exceeds the required level.  
% Additionally, we apply action post-processing to keep EV SoCs within valid boundaries by adjusting the power rate for stopping charging or discharging when they exceed $SoC^{\text{max}}(\phi(C_i, T_j))$ or drop below $SoC^{\text{min}}(\phi(C_i, T_j))$.  
We observe that off-peak hours offer lower electricity prices, enabling EV charging at higher power rates without affecting the final demand charge. This helps optimize EV charging during these periods, reducing energy costs and alleviating pressure during peak times. To implement this approach, we utilize a simple greedy method during off-peak hours, foregoing RL training during these times. EVs charge at maximum power until they reach their required SoC. Specifically, assuming the current time slot $T_j$ is within non-peak hours and EV $V' = \phi(C_i, T_j)$ is connected to charger $C_i$, if $\SOCR(V') < \SOC(V', T_j)$, then $P(C_i, T_j) = \min(C^{max}_i, (\SOCR(V') - \SOC(V', T_j)) \times {CAP}(V') / \delta)$. Discharging occurs if the SoC exceeds the required level, calculated as $P(C_i, T_j) = \max(C^{min}_i, (\SOCR(V') - \SOC(V', T_j)) \times {CAP}(V') / \delta)$.


To condense the state features while accounting for the common maximum and minimum SoC boundaries of all EVs (with $\SOCMIN=0$ and $\SOCMAX=90\%$), we do not include SoC boundaries in the state representation, limiting the policy's direct access to them for action control. To maintain valid SoC boundaries, we apply a post-processing procedure, which differs from action masking that is integrated with the actor network and influenced by training backpropagation. This action post-processing adjusts policy-generated actions before they are input to the environment, ensuring that charging stops when SoC exceeds $SoC^{\text{max}}$ and discharging halts if it drops below $SoC^{\text{min}}$. 
By employing this approach, we ensure that all policy-generated power rates for charging EVs remain within the defined SoC boundaries, thereby satisfying Constraints~(\ref{eq:soc_min}) and~(\ref{eq:soc_max}).
%This method allows the RL policy to concentrate on the objective of total bill reduction without needing to learn the validity of actions concerning SoC limits, thereby enhancing the effectiveness of the training process. 


